Explanation Needs in App Reviews: Taxonomy and Automated Detection

Explainability, i.e. the ability of a system to explain its behavior to users, has become an important quality of software-intensive systems. Recent work has focused on methods for generating explanations for various algorithmic paradigms (e.g., machine learning, self-adaptive systems). There is relatively little work on what situations and types of behavior should be explained. There is also a lack of support for eliciting explainability requirements. In this work, we explore the need for explanation expressed by users in app reviews. We manually coded a set of 1,730 app reviews from 8 apps and derived a taxonomy of Explanation Needs. We also explore several approaches to automatically identify Explanation Needs in app reviews. Our best classifier identifies Explanation Needs in 486 unseen reviews of 4 different apps with a weighted F-score of 86%. Our work contributes to a better understanding of users' Explanation Needs. Automated tools can help engineers focus on these needs and ultimately elicit valid Explanation Needs.

==> draft.tex <==
Fisher Test
%In addition, we conducted an evaluation of the datasets to determine the statistical significance of the variations in the proportion of explanation needs in app reviews across our different data sources. To this aim, we applied the two-sided Fisher's Exact Test. This test was appropriate as it can be used for contingency tables and returns exact p-values for small sample sizes \cite{sprent_fisher_2011}. 

%The results show that the difference in the proportions between \scrape and \ens, as well as between \scrape and \pbr, are highly significant ($p<0.01$) (see Figure~\ref{fig:fisher_test_diagram}). The effect size, expressed in odds-ratio, is greater than two for observing an explanation need in \scrape, compared to the \ens and \pbr. At the same time, the test reported no significant difference in the proportions of explanation need occurrences between \scrape and \pbr ($p=1$).

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=0.6\linewidth]{./figs/fisher_test_diagram.png}
%    \caption{\todo{rename datasets in the figure}Overview of Fisher's Exact Tests Between Data Sources}
%    \label{fig:fisher_test_diagram}
%\end{figure}



Thread to validity

\subsection{Threats to Validity}
%We have identified several threats to the validity of this part of our research, specifically potential threats to \textit{construct, internal and external validity}.
One possible threat to construct validity is that our concept of \emph{Explanation Needs} may exceed the traditional boundaries of the topic of explainability. This is due to the fact that we were unable to determine which specific \emph{Explanation Needs} could be logically translated into requirements for explainability, as there is insufficient information available to make such an assessment. In response to this, we have defined the term \emph{Explanation Needs} more broadly, which allowed us to take a more holistic perspective on people's overall needs for explanations.

Regarding the internal validity of our work, there are some potential threats that we need to consider. One such threat is using quantitative coding, which can be interpretive and subjective. This means that our analysis may be influenced by our own biases or assumptions, which could impact the accuracy of our findings.
Another potential threat is the issue of poor English and typing errors in some of the app reviews we analyzed. This could make it difficult or even impossible to fully comprehend the content of these reviews, which may result in inaccurate conclusions or interpretations.
However, to address this potential threat, we made a conscious effort to discuss and evaluate any incomprehensible reviews and either disregarded them or included them in our analysis only after careful consideration.

Lastly, a threat to external validity could be survivorship bias.
We need to consider the possibility that the explanation needs we identified in our study may not be representative of people with low technological literacy, as they may be less likely to write and publish app reviews in the first place. This may limit the generalizability of our findings to the broader population.
Furthermore, it is important to note that the app reviews we analyzed in our qualitative analysis were relatively old and low in number, with only a few cases of explanation needs observed. It means that the taxonomy categories we developed are based on a relatively small sample size of reviews. However, we took steps to mitigate this potential threat by ensuring that our coding process was thorough and saturated and by applying the same codes to an extended dataset to test their validity further.
Despite the potential limitations of our study, we believe that our findings provide valuable insights into the types of \emph{Explanation Needs} that app users may have.



==> tables/DS-1_ExpNeeds.tex <==

\begin{table}
\centering
\caption{Distribution of Explanation Needs types \ens Apps}
\label{tab:exp-needs}
\begin{tabularx}{\linewidth}{l*{6}{>{\centering\arraybackslash}X}}
\toprule
Name & Expl. Need & Tra & Int & Bus & Dis & Err \\
\midrule
Baby Tracker & 8 (4.0\%) & 3 & 1 & 1 & 3 & -- \\
Experian Credit & 10 (4.8\%) & -- & 5 & 1 & 3 & 1 \\
Follow My Health & 12 (5.2\%) & 4 & -- & 1 & 3 & 4 \\
Stock Master & 9 (4.0\%) & 3 & 2 & 1 & 3 & -- \\
Here We Go & 9 (4.1\%) & 1 & 1 & 1 & 3 & 3 \\
MiBand & 9 (4.1\%) & 2 & 2 & 1 & -- & 4 \\
Waze & 8 (3.6\%) & 1 & -- & -- & 4 & 3 \\
Yazio & 12 (5.8\%) & 3 & 2 & -- & 7 & -- \\
\midrule
Total & 77 (4.6\%) & 17 & 13 & 6 & 26 & 15 \\
& & 22.1\% & 16.9\% & 7.8\% & 33.8\% & 19.5\% \\
\bottomrule
\end{tabularx}
  \begin{acronym}
    {\scriptsize \acro{Tra:}{Training},  \hspace{1pt} \textbf{Int:} { Interaction},  \hspace{1pt}\textbf{Bus:} { Business},   \hspace{1pt}\textbf{Dis:} { Dissatisfaction},   \hspace{1pt}\textbf{Err:} { Errata} }
  \end{acronym}
\end{table}


==> tables/appReviewDS1.tex <==
\begin{table}
    \centering
    \caption{An overview of the apps whose reviews are included in our   \ens: }
    \label{tab:AppOverviewDS1}
    \begin{tabularx}{1 \linewidth}{l X l r@{}}
        \toprule
        Name & Description & Store & Size \\ \midrule
        Baby Tracker & Newborn Tracking & App Store & 200 \\
        Experian Credit & Credit Reporting & App Store & 210 \\
        Follow My Health & Patient Engagement & App Store & 229 \\
        Stock Master & Financial Trading & App Store & 226 \\
        Here We Go & Navigation Software & Google Play & 220 \\
        MiBand & Smartwatch Companion & Google Play & 217 \\
        Waze & Navigation Software & Google Play & 221 \\
        Yazio & Nutrition Tracking & Google Play & 207 \\ \midrule
        Total & & & 1730\\
        \bottomrule
    \end{tabularx}
\end{table}

==> tables/categoriesDS1.tex <==
\begin{table*}
    \centering
    \caption{An overview of the categories found in our   \ens: }
    \label{tab:categoryOverviewDS1}
    \begin{tabularx}{1 \linewidth}{l X l r r | r r r r r@{}}
        \toprule
        Name & Description & Store & Size & Expl. Need & Training & Interaction & Business & Dissatisfaction & Errata \\ \midrule
        Baby Tracker & Newborn Tracking & App Store & 200 & 8 (4.0\%) & 3 & 1 & 1 & 3 & - \\
        Experian Credit & Credit Reporting & App Store & 210 & 10 (4.8\%) & - & 5 & 1 & 3 & 1\\
        Follow My Health & Patient Engagement & App Store & 229 & 12 (5.2\%) & 4 & -& 1 & 3 & 4\\
        Stock Master & Financial Trading & App Store & 226 & 9 (4.0\%) & 3 & 2 & 1 & 3 & - \\
        Here We Go & Navigation Software & Google Play & 220 & 9 (4.1\%) & 1 & 1 & 1 & 3 & 3\\
        MiBand & Smartwatch Companion & Google Play & 217 & 9 (4.1\%) & 2 & 2 & 1 & - & 4\\
        Waze & Navigation Software & Google Play & 221 & 8 (3.6\%) & 1 & - & - & 4 & 3\\
        Yazio & Nutrition Tracking & Google Play & 207 & 12 (5.8\%) & 3 & 2 & - & 7 & -\\ \midrule
        Total & & & 1730 & 77 (4.6\%) & 17 & 13 & 6 & 26 & 15\\
        & & & & & 22.1\% & 16.9\% & 7.8\% & 33.8\% & 19.5\%\\
        \bottomrule
    \end{tabularx}
\end{table*}

==> tables/interRaterTaxonomy.tex <==
\begin{table*}
    \centering
    \caption{Inter-annotator agreement statistics in the taxonomy validation process}
    \label{tab:interRaterTaxonomy}
    \begin{tabular}{lrrrrrrrrrrrrr}
        \toprule
         &  & \multicolumn{2}{c}{Explanation Need}  & \multicolumn{2}{c}{Training} & \multicolumn{2}{c}{Errata} & \multicolumn{2}{c}{Dissatisfaction} & \multicolumn{2}{c}{Interaction} & \multicolumn{2}{c}{Business} \\
         & & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{1} & \textbf{0} & \textbf{1}\\
        Confusion Matrix & \textbf{0} & 63 & 7 & 55 & 4 & 56 & 4 & 51 & 4 & 52 & 12 & 70 & 0 \\
         & \textbf{1} & 53 & 77 & 4 & 14 & 5 & 12 & 10 & 12 & 3 & 10 & 2 & 5 \\ \midrule
         Agreement & & \multicolumn{2}{c}{70.0\%} & \multicolumn{2}{c}{89.6\%} & \multicolumn{2}{c}{88.3\%} & \multicolumn{2}{c}{81.8\%} & \multicolumn{2}{c}{80.5\%} & \multicolumn{2}{c}{97.4\%} \\
         Cohen's Kappa & & \multicolumn{2}{c}{0.427} & \multicolumn{2}{c}{0.710} & \multicolumn{2}{c}{0.653} & \multicolumn{2}{c}{0.515} & \multicolumn{2}{c}{0.456} & \multicolumn{2}{c}{0.820}\\
         Gwet's AC1 & & \multicolumn{2}{c}{0.403} & \multicolumn{2}{c}{0.838} & \multicolumn{2}{c}{0.824} & \multicolumn{2}{c}{0.711} & \multicolumn{2}{c}{0.700} & \multicolumn{2}{c}{0.970} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/sourceDescription.tex <==
\begin{table}
    \centering
    \caption{Data Source Description}
    \label{tab:DataSources}
    \begin{tabular}{@{}llr@{}}
        \toprule
        Name & Store & Size \\ \midrule
        \ens & App Store, Google Play & 1,730 \\
        \pbr & Google Play & 2,449 \\
        \scrape & App Store & 899 \\
        \DSFour & App Store, Google Play & 486 \\
        \bottomrule
    \end{tabular}
\end{table}
